CARE: Ensemble Adversarial Robustness Evaluation Against Adaptive Attackers for Security Applications

Ensemble defenses, are widely employed in various security-related applications to enhance model performance and robustness. The widespread adoption of these techniques also raises many questions: Are general ensembles defenses guaranteed to be more robust than individuals? Will stronger adaptive attacks defeat existing ensemble defense strategies as the cybersecurity arms race progresses? Can ensemble defenses achieve adversarial robustness to different types of attacks simultaneously and resist the continually adjusted adaptive attacks? Unfortunately, these critical questions remain unresolved as there are no platforms for comprehensive evaluation of ensemble adversarial attacks and defenses in the cybersecurity domain. In this paper, we propose a general Cybersecurity Adversarial Robustness Evaluation (CARE) platform aiming to bridge this gap.

==> 1.1-introduction.tex <==
\section{introduction}

Adversarial examples, inputs designed to induce worst-case behavior in machine learning models, have been extensively studied over the past decade.
In this paper, we propose a systematic approach to characterize worst-case (i.e., optimal) adversaries.
With our decomposition, we enumerate over components to create 576 attacks (568 of which were previously unexplored). Next, we propose the Pareto Ensemble Attack (PEA): a theoretical attack that upper-bounds attack performance.

% 自适应攻击下鲁棒集成防御提高了多少可证明鲁棒性
% 测试自适应攻击场景下经验鲁棒性和可证明鲁棒性的gap

% 可验证鲁棒性
% 集成模型的可验证鲁棒性很难量化

% Different defense approaches have been proposed against adversarial attacks, including: a) empirical defenses, which can usually be adaptively attacked again without providing robustness certiﬁcation; and b) certiﬁably robust approaches, which consist of robustness veriﬁcation providing the lower bound of robust accuracy against any attacks under certain conditions and corresponding robust training approaches.

% To defend against such attacks, there are several works proposed to empirically improve the robustness of DNNs [8],
% [16]–[20]. However, many of such defenses can be adaptively attacked again by sophisticated attackers [12], [21]. The everlasting competition between attackers and defenders motivates studies on the certiﬁably robust approaches for DNNs, which include both robustness veriﬁcation and robust training approaches [22]–[28]. The robustness veriﬁcation approaches aim to evaluate DNN robustness by providing a theoretically certiﬁed lower bound of robustness under certain perturbation constraints; the corresponding robust training approaches aim to train DNNs to improve such lower bound.

% Adaptive attacks have (rightfully) become the de facto standard for evaluating defenses to adversarial examples.
